On the Relationship Between Double Descent of CNNs and Shape/Texture Bias Under Learning Process

The double descent phenomenon, which deviates from the traditional bias-variance trade-off theory, attracts considerable research attention; however, the mechanism of its occurrence is not fully understood. On the other hand, in the study of convolutional neural networks (CNNs) for image recognition, methods are proposed to quantify the bias on shape features versus texture features in images, determining which features the CNN focuses on more. In this work, we hypothesize that there is a relationship between the shape/texture bias in the learning process of CNNs and epoch-wise double descent, and we conduct verification. As a result, we discover double descent/ascent of shape/texture bias synchronized with double descent of test error under conditions where epoch-wise double descent is observed. Quantitative evaluations confirm this correlation between the test errors and the bias values from the initial decrease to the full increase in test error. Interestingly, double descent/ascent of shape/texture bias is observed in some cases even in conditions without label noise, where double descent is thought not to occur. These experimental results are considered to contribute to the understanding of the mechanisms behind the double descent phenomenon and the learning process of CNNs in image recognition.

==> fig/fig_model_size_description.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{fig/fig_model_size.pdf}
\caption{
Learning process under various size conditions of ResNet family. Top: train/test errors Bottom: shape/texture bias values.}
\label{fig:comp_model}
\end{figure}

==> tab/tab_model_size.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{5pt}
\caption{Correlation coefficients and synchronization scores for different model sizes.}
\tablevspace
\scalebox{0.85}{
\begin{tabular}{c|ccc|ccc} 
\toprule
\multirow{2}{*}{Model} \tabletemplate \\
\midrule
ResNet18 &0.778&\textminus0.778 & 0.778 & \textminus0.026&0.118 & 0.072\\
ResNet34 &0.498& \textminus0.536 & 0.517 & 0.165 & \textminus0.281 & 0.223\\
ResNet50 &\textminus0.153&0.136& 0.144 & \textminus0.097&0.064 & 0.080\\
\bottomrule
\end{tabular}
}
\label{tab:model_size}
\end{table}

